Crumbling Abstract Machines

Extending the lambda-calculus with a construct for sharing, such as let expressions, enables a special representation of terms: iterated applications are decomposed by introducing sharing points in between any two of them, reducing to the case where applications have only values as immediate subterms. This work studies how such a crumbled representation of terms impacts on the design and the efficiency of abstract machines for call-by-value evaluation. About the design, it removes the need for data structures encoding the evaluation context, such as the applicative stack and the dump, that get encoded in the environment. About efficiency, we show that there is no slowdown, clarifying in particular a point raised by Kennedy, about the potential inefficiency of such a representation. Moreover, we prove that everything smoothly scales up to the delicate case of open terms, needed to implement proof assistants. Along the way, we also point out that continuation-passing style transformations--that may be alternatives to our representation--do not scale up to the open case.

==> 06-comments_on_related_works.tex <==
% !TEX root = main.tex
\section{Comments on Related Works}
\label{sect:kennedy-danvy}
Here we discuss in detail Kennedy's potential slowdown and provide a counter-example to the scalability of the CPS transformation to open \lat{s}.

\paragraph{Kennedy}
\newcommand{\toCC}{\to_{\mathtt{CC}}}
\newcommand{\MyBeta}{\betav}
\newcommand{\toMyBeta}{\to_{\MyBeta}}
\citet{DBLP:conf/icfp/Kennedy07} compares three different calculi: a monadic calculus, which has ES, a calculus of administrative normal forms (ANFs) and the image of a CPS transformation. 
In the monadic calculus $\betav$-redexes can be hidden by ES which need to be commuted to reveal the $\betav$-redex. 
Kennedy shows an example (Problem 2 of Section 2.3 in \citet{DBLP:conf/icfp/Kennedy07}, see \reffig{kennedy}) where the number of commutations is not bounded linearly by the number of $\betav$-steps and blames the inefficiency of his compiler on that. The offending term is the following:
\[
\tm \defeq \ (\varthree_1 \var_0) \,\esub{\varthree_1}{\la{\var_1} \consttwo\vartwo_1 \esub{\vartwo_1}{\varthree_2\var_1}} \,\esub{\varthree_2}{\la{\var_2} \consttwo\vartwo_2 \esub{\vartwo_2}{\varthree_3\var_2}} \dots \esub{\varthree_n}{\la{\var_n} \consttwo \vartwo_n \esub{\vartwo_n}{\consttwo\var_n}}.
\]

We include in \reffig{kennedy} Kennedy's example of a normalizing sequence for $\tm$ that has a number of commutations \emph{quadratic} in the number of $\betav$-steps. Here we actually denote by $\toMyBeta$ a $\to_{\elsym}$ step followed by a $\tobv$ step (similar respectively to $\beta$-\textsc{Let} and $\beta$-\textsc{Fun} in \citet{DBLP:conf/icfp/Kennedy07}).
The reduction sequence consists of single $\toMyBeta$ steps followed by a number of $\toCC$ steps; more precisely, the $i^\textup{th}$ $\MyBeta$-step is immediately followed by $i$ commutation steps $\toCC$, where each $\MyBeta$ step is a linear beta step performed in the body of the rightmost ES; \reffig{kennedy} explicitly shows how the $(i+1)^\textup{th}$ step is performed.


\begin{figure}[!ht]
%\scalebox{0.95}{
\begin{align*}
 \tm\quad &
 (\toMyBeta \toCC) \,\, (\toMyBeta \toCC^2) \,\cdots\, (\toMyBeta \toCC^i) \\ %= \toMyBeta^i \cup \toCC^{i(i+1)/2} \\
&(\varthree_1 \var_0) \esub{\varthree_1}{\la{\var_1} \consttwo\vartwo_1 \esub{\vartwo_1}{\varthree_2\var_1}} \esub{\varthree_2}{\la{\var_2} \consttwo\vartwo_2 \esub{\vartwo_2}{\varthree_3\var_2}} \dots \\
&\dots \esub{\varthree_{n-i-1}}{\la{\var_{n-i-1}} \consttwo \vartwo_{n-i-1} \esub{\vartwo_{n-i-1}}{\varthree_{n-i}\var_{n-i-1}}} \\
& \textcolor{white}{\ldots\ldots}\esub{\varthree_{n-i}}{\la{\var_{n-i}} \consttwo \vartwo_{n-i} \esub{\vartwo_{n-i}}{\consttwo \vartwo_{n-i+1}} \esub{\vartwo_{n-i+1}}{\consttwo \vartwo_{n-i+2}} \dots \esub{\vartwo_n}{\consttwo \var_{n-i}}}
\\
\toMyBeta \\
&(\varthree_1 \var_0) \esub{\varthree_1}{\la{\var_1} \consttwo\vartwo_1 \esub{\vartwo_1}{\varthree_2\var_1}} \esub{\varthree_2}{\la{\var_2} \consttwo\vartwo_2 \esub{\vartwo_2}{\varthree_3\var_2}} \dots \\
&\dots \esub{\varthree_{n-i-1}}{\la{\var_{n-i-1}} \consttwo \vartwo_{n-i-1} \esub{\vartwo_{n-i-1}}
{\consttwo \vartwo_{n-i} \esub{\vartwo_{n-i}}{\consttwo \vartwo_{n-i+1}} \esub{\vartwo_{n-i+1}}{\consttwo \vartwo_{n-i+2}} \dots \esub{\vartwo_n}{\consttwo \var_{n-i-1}}}}
\\
\toCC^{i+1} \\
&(\varthree_1 \var_0) \esub{\varthree_1}{\la{\var_1} \consttwo\vartwo_1 \esub{\vartwo_1}{\varthree_2\var_1}} \esub{\varthree_2}{\la{\var_2} \consttwo\vartwo_2 \esub{\vartwo_2}{\varthree_3\var_2}} \dots \\
&\dots \esub{\varthree_{n-i-1}}{\la{\var_{n-i-1}} \consttwo \vartwo_{n-i-1} \esub{\vartwo_{n-i-1}}{\consttwo \vartwo_{n-i}} \esub{\vartwo_{n-i}}{\consttwo \vartwo_{n-i+1}} \dots \\
&\dots \esub{\vartwo_n}{\consttwo \var_{n-i-1}}}
\end{align*}
%}
%\Description{Kennedy's example of evaluation in the monadic calculus where the number of commutation steps is quadratic in the number of $\betav$-steps.}
\caption{Kennedy's example of evaluation in the monadic calculus where the number of commutation steps is quadratic in the number of $\betav$-steps ($\to^i$ stands for the composition of $i$ $\to$-steps). 
The $i^\textup{th}$ $\betav$-step is immediately followed by %$i+1$ 
$i$ commutation steps $\toCC$ that just append two lists of substitutions moving one substitution at a time. 
Therefore, one needs $n$ $\betav$-steps and ${n(n+1)}/{2}$ $\toCC$-steps to reach the normal form.
In the %abnormal calculus
\Crumble and \oaglam instead, the commutation steps are integrated in the $\betav$-rule simply by appending the two lists in constant time.}
\label{fig:kennedy}
\end{figure}

ANFs are just canonical shapes of monadic terms where the topmost term and the body of each abstraction is a \crumblep, \ie a term together with a list of ES that map variables to terms (instead of \crumble{s}). 
Kennedy rightly observes that ANFs are not preserved by standard $\betav$-reduction and thus, after every $\betav$-step, some commutative steps are required to reach the ANF shape. 
The quadratic example by Kennedy stands in the ANF fragment. 
Therefore Kennedy too hastily concludes that the quadratic blowup also affects the ANF calculus.

However, Kennedy misses the fact that the ES in ANFs form a list and that the commutations steps altogether just implement the append function of two lists. Since append can be implemented in constant time, the complexity of evaluation in the ANF calculus is just linear (and not quadratic) in the number of $\betav$-steps. 
This is the same complexity we achieved %in our paper for the abnormal calculus
for the \Crumble and \oaglam. 


\paragraph{Danvy and Filinski}
 In \citet{DBLP:journals/mscs/DanvyF92} the CPS transformation is shown to scale up to open \lat{s} (their Theorem 2). 
 On open \lat{s}, however, they consider Plotkin's \cbv operational semantics $\plotcalc$, which is \emph{not adequate} (it is adequate only for closed terms, see \citet{DBLP:conf/aplas/AccattoliG16,aplas18}). 
 When one considers one of the equivalent adequate \cbv semantics in \citet{DBLP:conf/aplas/AccattoliG16,aplas18} for the open case, for instance the fireball calculus $\firecalc$, then the properties of the CPS no longer hold, in particular it does not commute with evaluation, as the following example shows.
Take the following open \lat $\tm \defeq (\la{\var} {\la{\vartwo}\vartwo}) (\varthree \varthree) \val$, where $\val$ is a \lav, say a distinguished variable.
 In $\plotcalc$ the \lat $\tm$ is $\betav$-normal, but in $\firecalc$ we have:
\begin{align*}
	\tm \defeq (\la{\var} {\la{\vartwo}\vartwo}) (\varthree \varthree) \val \tof (\la{\vartwo}{\vartwo})\val \tof \val
\end{align*}


Now, consider the CPS translation $\mathtt{cps}(\tm)$ of $\tm$, according to the definition in \citet{DBLP:journals/mscs/DanvyF92}.
We use $\lambda$ for standard (``dynamic'', in Danvy's terminology) abstraction, and $\Lambda$ and $@$ for ``static'' abstraction and application, respectively.
If a generalized version of Theorem 2 in \citet{DBLP:journals/mscs/DanvyF92} held in the open case, one would expect that $@ (\mathtt{cps}(\tm)) I$ (where $I \defeq \la{\varthree}\varthree$) evaluates %$@ (\mathtt{cps}(\val)) I$ (where $I \defeq \la{\varthree}\varthree$), and in particular 
to $\val$, as $\val$ is a variable.
But, even using an unrestricted $\beta$-reduction that goes under abstraction as evaluation, we obtain
%In the example we use $\lambda$ for standard (``dynamic'', in Danvy's terminology) abstraction, and $\Lambda$ and $@$ for ``static'' abstraction and application, respectively.
%Moreover we reduce at once all static redexes first, followed by all dynamic redexes.
(we reduce all static redexes first, followed by all dynamic redexes):

  \begin{align*}
%   &(\la{\var} {\la{\vartwo}\vartwo}) (\varthree \varthree) \val \tof (\la{\vartwo}{\vartwo})\val \tof \val \\~\\
%   &@\mathtt{cps}((\la{\var}{\la{\vartwo}\vartwo}) (\varthree \varthree) \val) I
   &@ (\mathtt{cps}(\tm)) I   \\= \ &(\Lambda k.
        @
         (\Lambda x.
           @
            (\Lambda y.
              @ y
               (\lambda w.
                 \lambda a.
                  @
                   (\Lambda b.
                     @ b
                      (\lambda c.
                        \lambda d.
                         @ (\Lambda e. @ e c) (\Lambda e. d e)))
                   (\Lambda b. a b)))\\~~~~
            &(\Lambda y.
              @
               (\Lambda w.
                 @ (\Lambda a. @ a z)
                  (\Lambda a.
                    @ (\Lambda b. @ b z)
                     (\Lambda b. (a b) (\lambda c. @ w c))))
               (\Lambda w. (y w) (\lambda a. @ x a))))\\~~~~~~
         &(\Lambda x.
           @ (\Lambda y. @ y v)
            (\Lambda y. (x y) (\lambda w. @ K w)))) I\\
   \tob^* \ &
   (\varthree\varthree)
    (\lambda x.
      ((\lambda y. \lambda w. w (\lambda a. \lambda b. b a)) x)
       (\lambda y. y v (\lambda w. I w)))\\
  \tob^* \ &
  (\varthree\varthree) (\la \var \val)
\end{align*}

\noindent
where $ (\varthree\varthree) (\la \var \val)$ is not even $\beta$-equivalent to $\val$.
The CPS translation---like Plotkin's calculus---gets stuck trying to evaluate $z z$, whereas the term reduces to $v$ in the fireball calculus.

Summing up, we are not claiming that Theorem~2 in \citet{DBLP:journals/mscs/DanvyF92} is false, but just that it does not mean that their CPS transformation %does not fully 
scale up to open \lat{s}:
to prove scalability, one should use an adequate \cbv evaluation for open \lat{s} (such as the one of the fireball calculus), instead of Plotkin's one.
Our counter-example shows that Danvy's and Filinski's CPS does not scale up to open \lat{s} with an adequate \cbv operational semantics for them.

It is worth noting that this problem affects also other CPS translations, such as the ones defined by \citet{DBLP:journals/tcs/Plotkin75} or by \citet{DBLP:conf/lics/Lassen05}. 
Likely, this is the reason why \citet{DBLP:conf/lics/Lassen05} states his Theorem 4.6 (the analogous of Theorem 2 in \citet{DBLP:journals/mscs/DanvyF92}) only for closed \lat{s}.

==> image_easy_glamour.tex <==
% !TEX root = main.tex
\begin{figure}[t]
\begin{center}
$\begin{array}{c}
\textsc{Grammars}
\\
\begin{array}{r\colspace \colspace rclcrrlllllllll}
	\textsc{Values} & \val 	& \grameq & \la\var\code
	\\
       
	\textsc{Stacks} & \stack 	& \grameq & \stempty \mid \val \cons \stack
	\\
	\textsc{Global env.} & \genv	& \grameq & \stempty \mid \esub\var\val \!\cons\! \genv 
	\\
	\textsc{Dumps} &	\dump	& \grameq & \stempty \mid \dump \cons \dentry\code\stack 
	\\
	\textsc{States} &	\state	& \defeq & \glamst\dump\code\stack\genv
\end{array}
\\\\

\textsc{Transitions}
\\
  	{\setlength{\arraycolsep}{0.35em}
  	\begin{array}{c|c|c|c|c|c|c|c|ccc}
		\mbox{Dump} & \mbox{Code} & \mbox{Stack} & \mbox{Global Env} 
		&&
		\mbox{Dump} & \mbox{Code} & \mbox{Stack} & \mbox{Global Env}\\
\hhline{=|=|=|=|=|=|=|=|=}
		\dump & \code\codetwo & \stack & \genv
	  	&\tomachcone&
	  	\!\dump\!\cons\!\dentry\code\stack\! & \codetwo & \stempty &\genv
	  	\\
%\hhline{-|-|-|---|-|-|-}
		\!\dump\!\cons\!\dentry\code\stack\! & \la\var\codetwo & \stempty & \genv
		& \tomachctwo &
		\dump & \code & \la\var\codetwo \cons\stack & \genv
		\\

		\dump & \la\var\code & \val\!\cons\!\stack & \genv
	  	&\tomachbeta &
		\dump & \code & \stack & \esub\var\val\genv
	  	\\

	  	\dump & \var & \stack & \genv_1\esub\var\val\genv_2
		& \tomachvar &
		\dump & \!\rename{\val}\! & \stack & \genv_1\esub\var{\val}\genv_2\\

	\end{array}}
\\\\
\mbox{where $\rename{\val}$ is any well-named code $\alpha$-equivalent to $\val$ such that its }
\\ \mbox{bound names  are fresh with respect to those in $\dump$, $\stack$ and $\genv_1 \esub\var\val \genv_2$.}
\end{array}
$
  \end{center}
  \caption{\label{fig:glam} The GLAM}
\end{figure}

==> table-ocaml-glam.tex <==
\begin{table}
  \begin{lstlisting}
type var =
 { mutable content: [ `Shared of term | `Copied of var | `None ] }
and term =
| Var of var
| Abs of var * term
| App of term * term

let mk_var content = { content }

let copying x x' f =
 let saved = x.content in
 x.content <- `Copied x' ;
 let res = f () in
 x.content <- saved ;
 res

let rec copy =
 function
 | App(t1,t2) -> App(copy t1, copy t2)
 | Abs(x,t) ->
   let x' = mk_var `None in 
   let t' = copying x x' (fun _ -> copy t) in
   Abs(x', t')
 | Var {content = `Copied v} -> Var v
 | Var _ as t -> t

let eval =
 let rec aux d s t = match d, s, t with
 | _, _, App(t1,t2) -> aux ((t1, s)::d) [] t2 (* c1 *)
 | (u,s) :: d, [], Abs _ -> aux d (t::s) u (* c2 *)
 | _, v::s, Abs(x,t) -> x.content <- `Shared v ; aux d s t (* r_beta *)
 | _, _, Var {content = `Shared v} -> aux d s (copy v) (* var *)
 | _, _, Var {content = `Copied _} -> assert false
 | _, _, Var {content = `None} -> failwith "Open"
 | [], [], Abs _ -> t
 in aux [] []
 \end{lstlisting}
  \caption{OCaml implementation of the GLAM}
\end{table}

